Volumetric Attribute Compression for 3D Point Clouds using Feedforward Network with Geometric Attention

We study 3D point cloud attribute compression using a volumetric approach: given a target volumetric attribute function $f : \mathbb{R}^3 \rightarrow \mathbb{R}$, we quantize and encode parameter vector $\theta$ that characterizes $f$ at the encoder, for reconstruction $f_{\hat{\theta}}(\mathbf{x})$ at known 3D points $\mathbf{x}$'s at the decoder. Extending a previous work Region Adaptive Hierarchical Transform (RAHT) that employs piecewise constant functions to span a nested sequence of function spaces, we propose a feedforward linear network that implements higher-order B-spline bases spanning function spaces without eigen-decomposition. Feedforward network architecture means that the system is amenable to end-to-end neural learning. The key to our network is space-varying convolution, similar to a graph operator, whose weights are computed from the known 3D geometry for normalization. We show that the number of layers in the normalization at the encoder is equivalent to the number of terms in a matrix inverse Taylor series. Experimental results on real-world 3D point clouds show up to 2-3 dB gain over RAHT in energy compaction and 20-30% bitrate reduction.

==> implement_old.tex <==
\subsection{Inverse and square root inverse approximation}\label{subsec:inv_approx}

% Let first re-visit finite Taylor series expansion to approximate a real function $f: \mathbb{R} \rightarrow \mathbb{R}$:
% $$
%     f(x) \approx f(a) + \sum_{k=1}^{K} \frac{f^{(n)}(a)}{k!} (x - a)^k
% $$

% We use the above to approximate the inverse function $f_{inv}(x) &=& x^{-1}$ and the inverse square root function $f_{sqrtinv}(x) &=& x^{-\frac{1}{2}}$:
% \begin{align}
%     \hat{f}_{inv}(x, a) &= a^{-1} + \sum_{k=1}^{K} a^{-k}(a-x)^k  \\
%     \hat{f}_{sqrtinv}(x, a) &= a^{-\frac{1}{2}} + \sum_{k=1}^{K} \frac{1...(2k-1)}{2^k k!}  a^{-\frac{1}{2}-k} (a - x)^k
% \end{align}
% By let $\mu = \frac{1}{2a}$ we have the following instead:
% \begin{align}
%     \hat{f}_{inv}(x, \mu) &=  2\mu \left[ 1 + \sum_{k=1}^{K} (1-2\mu x)^k \right]\\
%     \hat{f}_{sqrtinv}(x, \mu) &= \sqrt{2\mu} \left[ 1 + \sum_{k=1}^{K} \frac{1...(2k-1)}{2^k k!} (1- \sqrt{2\mu}x)^k \right]
% \end{align}

Any invertible \red{positive definite and symmetric?} square matrix $\mathbf{X} \in \mathbb{R}^d \times \mathbb{R}^d$ can be eigen-decomposed as $\mathbf{X} = \mathbf{U} \bLambda \mathbf{U}^\top$, and the inverse and square root inverse of $\mathbf{X}$ can be exactly calculated as below.
% by applying $f_{inv}(x)$ and $f_{sqrtinv}(x)$ as below. 
\begin{align}
    \mathbf{X}^{-1} &=\mathbf{U} \mathbf{\Lambda}^{-1} \mathbf{U}^\top \\
    \mathbf{X}^{-\frac{1}{2}} &=\mathbf{U} \mathbf{\Lambda}^{-\frac{1}{2}} \mathbf{U}^\top
\end{align}

Using this fact, we use the finite Taylor series as the approximation of  $\hat{f}_{inv} \approx x^{-1}$ and $\hat{f}_{sqrtinv} \approx x^{-\frac{1}{2}}$ on $\bLambda$ instead and re-derive an approximation procedure for inverse and square root inverse, which does not require any eigen-decomposition, \ie,  
\begin{align}
    \mathbf{X}^{-1} &\approx \mathbf{U} \hat{f}_{inv}(\mathbf{\Lambda}, \mu) \mathbf{U}^T 
    % &\approx 2\mu \mathbf{U} \left[ 1 + \sum_{k=1}^{K} (1-2\mu \mathbf{\Lambda})^k \right] \mathbf{U}^T \\ 
    &\approx 2\mu \left[ \mathbf{I} + \sum_{k=1}^{K} (\mathbf{I}-2\mu \mathbf{X})^k \right] . \label{eq:inv_approx}
\end{align}
Then, given any vector $\mathbf{v} \in \mathbb{R}^d$, $\mathbf{X}^{-1}\mathbf{v}$ can be approximated as
\begin{align}
    \mathbf{X}^{-1} \mathbf{v} \approx 2\mu \left[ \mathbf{v} + \sum_{k=1}^{K} (\mathbf{I}-2\mu \mathbf{X})^k\mathbf{v} \right] \label{eq:inv_approx_vector}
\end{align}
We use same method to approximate the square root inverse of $\mathbf{X}$
\begin{align}
    \mathbf{X}^{-\frac{1}{2}} \mathbf{v} \approx \sqrt{2\mu} \left[ \mathbf{v} + \sum_{k=1}^{K} \frac{1...(2k-1)}{2^k k!} (\mathbf{I}- \sqrt{2\mu} \mathbf{X})^k\mathbf{v} \right] \label{eq:sqrtinv_approx_vector}
\end{align}
The eq.(\ref{eq:inv_approx_vector}) and eq.(\ref{eq:sqrtinv_approx_vector}) can be expressed simply as re-applying the \textit{same} feed forward layer multiple times with skip connection. Thus is illustrated in fig.(\ref{fig:taylor_expansion_block_diagram}) below.

As we can see, for eq.(\ref{eq:inv_approx_vector}) to converge, we need $(\mathbf{I}-2\mu \mathbf{X})^k \rightarrow 0$ as $k \rightarrow \infty$. Hence, $\mu$ much be set to appropriate value so that the spectral radius of of $\mathbf{L} = \mathbf{I}-2\mu \mathbf{X}$ much less than $1$. Hence we consider $\mu$ as hyperparameter for tunning later on.

% \textcolor{red}{[Thuc] Above, we relace $a = \frac{1}{2\mu}$, and we set $\mu$ close to $\frac{1}{\lambda_{max}(\mathbf{X})}$ in our work. This is why I think our approximation will start around $a$ which close to and greater than $\frac{\lambda_{max}(\mathbf{X})}{2}$. Depend on the the distribution of our eigenvalues, $a$ could be far to the right of the $\frac{1}{x}$ curve. Since the rest of the  eigenvalues might less than $\frac{\lambda_{max}(\mathbf{X})}{2}$ a lot, }

\subsection{Encoding flow}
As describe earlier, we define our basis at the finest level of detail $L$ in a way such that $\bPhi_L^\top \bPhi_L = \M$, where $\M$ is a identity matrix. Hence, we then have the following:
\begin{align}
    F_L^* = \Tilde{F}_L^* = \mathbf{y} 
\end{align}
where $\mathbf{y} = [f(\mathbf{x}_i)]$ is the column vector of samples of the
function f on the point cloud. Then from level $l=L-1$ to $l=0$, we use eq.(\ref{eqn:analysis_lowpass}) to derive the un-normalized coefficients $\Tilde{F}_l^*$ as below:
\begin{align}
    \Tilde{F}_l^* = \mathbf{A}_l \Tilde{F}_{l+1}^*
\end{align}
where $\mathbf{A}$ is a pre-defined sparse convolution operation (which we give detail in the section \ref{sec:results}). Noted here is that we could then calculate the normalized coefficients $F_l^* = (\bPhi_l^\top \bPhi_l)^{-1} \Tilde{F}_l^*$ by using the approximation of inverse in sec.(\ref{subsec:inv_approx}), where the operation $\bPhi_l^\top \bPhi_l$ is calculated using \eqref{eqn:PhiTPhi}. 

As we have $\mathcal{F}_{\ell+1}=\mathcal{F}_\ell\oplus\mathcal{G}_\ell$, so that  $f_{\ell+1}^*\in \mathcal{F}_{\ell+1}$ can be written as a linear combination of the basis functions $\Phi_\ell$ and $\Psi_\ell$,
\begin{align}
    f_{\ell+1}^* &= \bPhi_l F_l^* + \bPsi_l G_l^*. \\
    \Leftrightarrow \bPhi_{l+1} F_{l+1}^* &= \bPhi_l F_l^* + \bPsi_l G_l^* \\
    \Leftrightarrow \bPsi_l G_l^* &= \bPhi_{l+1} (F_{l+1}^* - \mathbf{A}_l^TF_l^*) \\
    \Leftrightarrow g_l^* &= \bPhi_{l+1} \delta F_{l+1}^*
\end{align}
Hence, the un-normalized highpass coefficients can be calculated as below:
\begin{align}
    \Tilde{G}_l^* &= (\bPsi_{l}^{\top} \bPsi_{l})G_l^* \\
    &= (\bPsi_{l}^{\top} \bPsi_{l}) (\bPsi_{l}^{\top} \bPsi_{l})^{-1} \bPsi_{l}^{\top}g^*_l \label{eq:replace_psi}  \\
    &= \mathbf{Z}_l \bPhi_{l+1}^T g_l^* \\
    &= \mathbf{Z}_l \bPhi_{l+1}^T\bPhi_{l+1} \delta F_{l+1}^* \\
    % &= \mathbf{Z}_l \bPhi_{l+1}^T\bPhi_{l+1} (F_{l+1}^* - \mathbf{A}_l^TF_l^*) \\
    % &= \mathbf{Z}_l (\bPhi_{l+1}^T\bPhi_{l+1}) \delta F_{l+1}^* \\
    % &= \tilde{\mathbf{Z}}_l (\bPhi_{l+1}^T\bPhi_{l+1})^{-1}(\bPhi_{l+1}^T\bPhi_{l+1}) \delta F_{l+1}^*\\
    &= \tilde{\mathbf{Z}}_l \delta F_{l+1}^*
\end{align}
Where as defined above, 
\begin{align}
    \tilde{\mathbf{Z}}_l^\top &= \left[\begin{array}{c}
        -(\A_l^a)^{-1}\A_l^{b\top} \\ 
        \I^b
    \end{array}\right] \\
    \Leftrightarrow \tilde{\mathbf{Z}}_l &= \left[\begin{array}{cc}
        -(\A_l^{b\top})^T(\A_l^a)^{-T} &\I^b
    \end{array}\right]
\end{align}
The operation above can be understood by seeing how it apply on vector $\delta F_{l+1}^* = F_{l+1}^* - \mathbf{A}_l^TF_l^*$:
\begin{align}
    \Tilde{G}_l^* = \delta F_{l+1}^{*b} - (\A_l^{b\top})^T(\A_l^a)^{-T}\delta F_{l+1}^{*a}
\end{align}
We can see now that the operation basically pick a subset $b$ coefficients of $\delta F_{l+1}^*$ minus a linear combination of a subset $a$ coefficients of $\delta F_{l+1}^*$, where $(\A_l^a)^{-1}$ can be approximated as described in sec.(\ref{subsec:inv_approx}). 

To calculate the orthogonal normalized highpass coefficients $\bar{G}_l^*$, we apply the operation $(\bPsi_l^T\bPsi_l)^{-\frac{1}{2}}$ to $\Tilde{G}_l^*$, where $\bPsi_l^T\bPsi_l = \mathbf{Z}_l \bPhi_{l+1}^T\bPhi_{l+1} \mathbf{Z}_l^T$.
\begin{equation}
    \bar{G}_l^* = (\bPsi_l^T\bPsi_l)^{-\frac{1}{2}} \Tilde{G}_l^*.
\end{equation}
Even though what we describe here is for orthogonal critical residual coding, for the non-critical residual coding, the calculation of highpass coefficients can be done similarly by expressing $g_\ell^* \in \cG_l \subset \cF_{l+1}$ in the basis $\bPhi_{\ell+1}$ instead, this will give overcomplete highpass coefficient $\Tilde{G}_l^* = (\bPhi_{l+1}^T\bPhi_{l+1}) \delta F_{l+1}^*$ which can be orthogonalized and normalized by $(\bPhi_{l+1}^T\bPhi_{l+1})^{-\frac{1}{2}}$. 

Hence, by the end of the encoding flow, we will have sets of coefficients $\bar{F}_0^*, \bar{G}_1^*, ..., \bar{G}_l^*, ... \bar{G}_{L-1}^*$ that corresponding to orthogonal sets of basis function $\bar{\bPhi}_0, \bar{\bPsi}_1, ... \bar{\bPsi}_l, ..., \bar{\bPsi}_{L-1}$ (or overcomplete sets basis $\bar{\bPhi}_0, ..., \bar{\bPhi}_l, ..., \bar{\bPhi}_L$ functions in non-critical case)

\subsection{Decoding flow}

As we know, the projected function $f_{\ell+1}^*\in \mathcal{F}_{\ell+1}$ can be reconstructed by $f_{\ell}^*$ and $g_{\ell}^*$
\begin{align}
    f_{\ell+1}^* &= f_{\ell}^* + g_{\ell}^* \\    
    \bPhi_{l+1} F_{l+1}^* &= \bPhi_l F_l^* + \bPsi_l G_l^*. \\
    \Leftrightarrow \bPhi_{l+1}^T\bPhi_{l+1} F_{l+1}^* &= \bPhi_{l+1}^T\bPhi_{1+1} \mathbf{A}_l^T F_l^* + \bPhi_{l+1}^T\bPhi_{l+1} \mathbf{Z}_l^T G_l^*. \\ 
    \Leftrightarrow F_{l+1}^* &= \mathbf{A}_l^T F_l^* + \mathbf{Z}_l^T G_l^*. \label{eq:reconstruct_F_lp1}
\end{align}

In sum, the reconstruction is performed as follows:  Starting at the coarsest level of detail $l=0$, recover $\bar{F}_0^*$, and set
\begin{equation}
    F_0^* = (\Phi_0^*\Phi_0)^{-\frac{1}{2}}\bar{F}_0^* .
\end{equation}

Then for $l=0$ to $l=L-1$, recover $\bar{G}_l^*$ and perform
\begin{equation}
    G_\ell^* = (\Psi_l^T\Psi_l)^{-1/2} \bar{G}_\ell^*
\end{equation}
Then use \eqref{eq:reconstruct_F_lp1} to reconstruct the higher level of detail. Finally, declare
\begin{equation}
    \hat{y} = F_L^* .
\end{equation}

\subsection{Basis functions scaling}
During our experiments, we noted that the inverse and square root inverse approximation will converge faster if all the basis functions have unit $\ell_2$ norm, i.e, $\bPhi^T\bPhi$ and $\bPsi^T\bPsi$ have $1$ along their diagonal. Hence, we now introduce a simple scaling operation at each level of detail $l$.
\begin{align}
    \mathbf{D}_{\bPhi_l} &= \textit{Diag}( \bPhi_l^T\bPhi_l) \\
    \mathbf{D}_{\bPsi_l} &= \textit{Diag}( \bPsi_l^T\bPsi_l)
\end{align}
And then incorporate these scaler into $\mathbf{A}_l$ and $\mathbf{Z}_l$ as follow:
\begin{align}
    \mathbf{A}'_l &= \mathbf{D}_{\bPhi_{l}}^{-\frac{1}{2}} \mathbf{A}_l \mathbf{D}_{\bPhi_{l+1}}^{\frac{1}{2}} \\
    \mathbf{Z}'_l &= \mathbf{D}_{\bPsi_{l}}^{-\frac{1}{2}} \mathbf{Z}_l
\end{align}
The result sparse convolution operation $\mathbf{A}'_l$ will guarantee that the basis function at each level of detail will have unit $\ell_2$ norm. Noted here that to calculate $\mathbf{D}_{\bPsi_l}$, we have to calculate $\mathbf{D}_{\bPhi_l}$ first to figure out $\mathbf{A}'_l$ so that $\mathbf{Z}_l$ can be calculated base on eq.\eqref{eq:define_ZT}. Having defined $\mathbf{Z}_l$, the norm of highpass basis function $\mathbf{D}_{\bPsi_l}$ can then be calculated as the diagonal of $\mathbf{Z}_l \bPhi_{l+1}^T\bPhi_{l+1} \mathbf{Z}_l^T$.
